Low-Cost and High-Throughput Testing of COVID-19 Viruses and Antibodies via Compressed Sensing: System Concepts and Computational Experiments

Coronavirus disease 2019 (COVID-19) is an ongoing pandemic infectious disease outbreak that has significantly harmed and threatened the health and lives of millions or even billions of people. COVID-19 has also negatively impacted the social and economic activities of many countries significantly. With no approved vaccine available at this moment, extensive testing of COVID-19 viruses in people are essential for disease diagnosis, virus spread confinement, contact tracing, and determining right conditions for people to return to normal economic activities. Identifying people who have antibodies for COVID-19 can also help select persons who are suitable for undertaking certain essential activities or returning to workforce. However, the throughputs of current testing technologies for COVID-19 viruses and antibodies are often quite limited, which are not sufficient for dealing with COVID-19 viruses' anticipated fast oscillating waves of spread affecting a significant portion of the earth's population. In this paper, we propose to use compressed sensing (group testing can be seen as a special case of compressed sensing when it is applied to COVID-19 detection) to achieve high-throughput rapid testing of COVID-19 viruses and antibodies, which can potentially provide tens or even more folds of speedup compared with current testing technologies. The proposed compressed sensing system for high-throughput testing can utilize expander graph based compressed sensing matrices developed by us \cite{Weiyuexpander2007}.

==> bibli.tex <==
\begin{thebibliography}{10}

\bibitem{eldar2012compressed}
YC Eldar, G Kutyniok, Compressed Sensing: Theory and Applications (Cambridge University Press, 2012).

\bibitem{candes2005decoding}
EJ Cand{\`e}s, T Tao, Decoding by linear programming.
\newblock IEEE Trans. Inf. Theory. 51(12):4203--4215 (2005).

\bibitem{d2011testing}
A d'Aspremont, L El~Ghaoui, Testing the nullspace property using semidefinite programming.
\newblock Math. prog. 127(1), 123-144 (2011).

\bibitem{candes2006robust}
EJ Cand{\`e}s, J Romberg, T Tao, Robust uncertainty principles: exact signal reconstruction from highly incomplete frequency information.
\newblock IEEE Trans. Inf. Theory. 52(2), 489-509 (2006).

\bibitem{candes2006stable}
EJ Cand{\`e}s, J~Romberg, T~Tao, Stable signal recovery from incomplete and inaccurate measurements.
\newblock Comm. on pure and appl. math. 59(8), 1207-1223 (2006).

\bibitem{donoho2005neighborly}
D~Donoho, Neighborly polytopes and sparse solution of underdetermined linear equations.
\newblock Technical report (Stanford University. Dept. of Statistics 2005).

\bibitem{Tillmann2014Computational}
AM Tillmann, ME Pfetsch, The computational complexity of the restricted isometry property, the nullspace property, and related concepts in compressed sensing.
\newblock IEEE Trans. Inf. Theory. 60(2), 1248-1259 (2014).

\bibitem{juditsky2011verifiable}
A~Juditsky, A~Nemirovski, On verifiable sufficient conditions for sparse signal recovery via $\ell_1$ minimization.
\newblock Math. prog. 127(1), 57-88 (2011).

\bibitem{cohen2009compressed}
A~Cohen, W~Dahmen, R~DeVore, Compressed sensing and best $k$-term approximation.
\newblock J. American Math. Soc. 22(1),211-231 (2009).

\bibitem{xu2011precise}
W~Xu, B~Hassibi, Precise stability phase transitions for $\ell_1$ minimization: a unified geometric framework.
\newblock IEEE Trans. Inf. Theory. 57(10), 6894-6919 (2011).

\bibitem{lee2008computing}
K~Lee, Y~Bresler, Computing performance guarantees for compressed sensing.
\newblock In Proceedings of IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP) (2008), pp. 5129-5132.

\bibitem{tang2011verifiable}
G~Tang, A~Nehorai, Verifiable and computable $\ell_\infty$ performance evaluation of $\ell_1$ sparse signal recovery.
\newblock In Proceedings of Conference on Information Sciences and Systems (CISS) (2011), pp. 1-6.

\bibitem{cho2013new}
M~Cho, W~Xu, New algorithms for verifying the null space conditions in compressed sensing.
\newblock In Proceedings of Asilomar Conference on Signals, Systems and Computers (2013), pp. 1038-1042.

\bibitem{xu2011Compressive}
W~Xu, E~Mallada, A~Tang, Compressive sensing over graphs.
\newblock In Proceedings of IEEE International Conference on Computer Communizations (INFOCOM) (2011), pp. 2087-2095.

\bibitem{firooz2010network}
MH Firooz, S~Roy, Network tomography via compressed sensing.
\newblock In Proceedings of IEEE Global Telecommunications Conference
  (GLOBECOM) (2010), pp. 1-5.

\bibitem{coates2001network}
MJ Coates, RD Nowak, Network tomography for internal delay estimation.
\newblock In Proceedings of IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP) (2001), vol. 6, pp. 3409-3412.

%\bibitem{wozencraft1961sequential}
%J~Wozencraft, B~Reiffen, Sequential Decoding (Technology Press of the Massachusetts Institute of Technology and Wiley, 1961).

%\bibitem{xu2004computationally}
%W~Xu, Y~Wang, Z~Zhou, J~Wang, A computationally efficient exact {ML} sphere decoder.
%\newblock In Proceedings of IEEE Global Telecommunications Conference
%  (GLOBECOM) (2004), pp. 2594-2598.

%\bibitem{Yu1993more}
%B~Yu, B~Yuan, A more efficient branch and bound algorithm for feature selection.
%\newblock Pat. Recognition 26(6), 883-889 (1993).

\bibitem{cvx}
M~Grant, S~Boyd, {CVX}: Matlab software for disciplined convex programming,
  version 2.1 beta.
\newblock \url{http://cvxr.com/cvx} (2012).

\bibitem{mosek}
{MOSEK ApS}, The MOSEK optimization toolbox for MATLAB manual. Version 7.1
  (Revision 31).
\newblock \url{http://docs.mosek.com/7.1/toolbox/index.html} (2015).

\bibitem{tsang2003network}
Y~Tsang, M~Coates, RD Nowak, Network delay tomography.
\newblock IEEE Trans. Signal Process. 51(8), 2125-2136 (2003).

\bibitem{vardi1996network}
Y~Vardi, Network tomography: estimating source-destination traffic intensities from link data.
\newblock J.American Stat. Assoc. 91(433), 365-377
  (1996).

\bibitem{castro2004network}
R~Castro, M~Coates, G~Liang, R~Nowak, B~Yu, Network tomography: recent developments.
\newblock Stat. Sci. 19(3), 499-517 (2004).

\bibitem{donoho2010precise}
DL~Donoho, J~Tanner, Precise Undersampling Theorems.
\newblock Proc. IEEE 98(6), 913-924 (2010).

\bibitem{brassard1996fundamentals}
G~Brassard, P~Bratley, Fundamentals of algorithmics (Englewood Cliffs: Prentice Hall, 1996).

\bibitem{wilson1996generating}
DB~Wilson, Generating random spanning trees more quickly than the cover time.
\newblock In Proceedings of the twenty-eighth annual ACM symposium on Theory of computing (1996), pp. 296-303.

\bibitem{matlabOOP}
Mathworks, Object-Oriented Programming in MATLAB. Retrieved May 26, 2017, from {https://www.mathworks.com/discovery/object-oriented-programming.html}

\end{thebibliography}
